Voicify Your UI: Towards Android App Control with Voice Commands

Nowadays, voice assistants help users complete tasks on the smartphone with voice commands, replacing traditional touchscreen interactions when such interactions are inhibited. However, the usability of those tools remains moderate due to the problems in understanding rich language variations in human commands, along with efficiency and comprehensibility issues. Therefore, we introduce Voicify, an Android virtual assistant that allows users to interact with on-screen elements in mobile apps through voice commands. Using a novel deep learning command parser, Voicify interprets human verbal input and performs matching with UI elements. In addition, the tool can directly open a specific feature from installed applications by fetching application code information to explore the set of in-app components. Our command parser achieved 90\% accuracy on the human command dataset. Furthermore, the direct feature invocation module achieves better feature coverage in comparison to Google Assistant. The user study demonstrates the usefulness of Voicify in real-world scenarios.

==> Evaluation.tex <==
\begin{table}[]
\begin{tabular}{cccc}
\hline
\textbf{Hit rate@k} & \textbf{No of Success} & \textbf{No of Fail} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Percentage\\  of Success\end{tabular}}} \\ \hline
\textit{k = 1} & 38 & 12 & 76\% \\ 
\textit{k = 3} & 41 & 9 & 82\% \\ \hline
\end{tabular}
\caption{The experiment results with k = 1 and k = 3 for 50 test cases.}
\label{table:result}
\end{table}

==> Usecases.tex <==
\section{A Use Case Scenario}
\label{sec:usecases}

In this section, we use the example in Fig.~\ref{fig:thumbnail_image} to demonstrate how \tool is useful in real-world scenario. The example includes usages of both direct feature invocation and background virtual assistant to completely replace physical interactions, which also applies to many other circumstances.

Cindy, as a mom of two kids, always has her hands busy with multiple tasks from cooking to cleaning all day long. As Cindy is passionate about cooking for her children, she often reaches out to her phone when preparing the meal to check for cooking ingredients and instructions. However, it is quite inconvenient for her to pick up the phone as her hands are often occupied when holding kitchen accessories. In addition, uncleanliness is a major concern to her hence she has to wash and dry her hands before and after touching the phone screen. Sometimes, her cooking glove prevents her from tapping on the screen or causing her to make imprecise tap. The whole cooking process is exhausted and unproductive, and she faced the same issue every day.

Cindy is introduced to \tool, and quickly learned how to use the tool effectively. When cooking, Cindy can entirely use her voice to navigate between different apps in the smartphone. With other virtual assistant such as Voice Access, Cindy would have to navigate through many screens with multiple interaction to view her saved recipes. Using \tool, she can directly view all her saved recipes in the World Cuisines app with a single voice command, hence saving a lot of time and efforts. For choosing the Healthy Burger recipe, she can provide short-form command "Press Healthy Burger", \tool will virtually tap on desire UI element and provide her with audio feedback. 


==> formativeStudy.tex <==
\section{Formative Study}
\label{sec:study}

Although voice assistant technology has been increasingly helpful for users with certain conditions, it is critical to understand the applicability of the technology for normal users and fathom the full utilization of the technology as a common way of human-computer interaction. To better comprehend the usage of voice control technology, we conducted a semi-structured interview with 14 participants, ranging from 21-28 years old. All participants view smartphones as indispensable and use technological devices regularly. We introduced the participants to Google Voice Access, which is the official Android tool that allows users to interact and control the device with spoken commands. We let the participants get accustomed to the tool and explore the installed applications on the phone, guided by Voice Access’s tutorial. We observe users’ activities during the experiment and collect participants’ opinions about Voice Access and virtual assistant to devise the design implications for \tool. The main focuses of this study are to i) identify the situations where a voice assistant is useful, ii) determine the tasks that participants commonly achieved using voice assistant, and iii) understand the challenges that users encountered when using the existing voice assistants.


\subsection{Findings}

Overall, participants expressed great excitement when controlling the mobile device with voice commands. Participants who had never used voice assistants before mentioned that ``voice controlling was more interesting than what I thought''. Other participants who have some experience with other voice assistants were also amazed by the capability to fully interact with on-screen elements using voice commands. Users suggested that they will start using voice control systems in the future. However, there are still some problems that affect the usability of the existing solution. We summarized major findings from the participants’ feedback and observations during the experiment.

\textit{Complex usage scenarios require a comprehensible system.}
 In terms of possible use cases of Voice Access, interviewees suggested daily circumstances such as showering, cooking and working. P1 and P4 mentioned that they would use Voice Access when the device is out-of-reach, while P2 and P5 noted that Voice Access would be helpful when ``their hand is busy with other activities''. Hence, it is induced that when users are focusing on their primary activity, the voice command system is the common choice to interact with mobile devices to perform a secondary activity. In addition, we noticed a steep learning curve when introducing Voice Access to the participants, as they found it challenging to recall the correct phrase structure to perform certain functions facilitated by the voice assistant. This was evident in participants revisiting the Voice Access tutorial multiple times when carrying out the experiment. P8 mentioned that ``some introduced functionalities are not functional or applicable'' when using the system, adversely influencing users’ confidence. Therefore, unnecessarily complications in usability will impede the transition toward wide adoption of voice control.

\textit{Usefulness of providing in-app feature shortcuts to improve usage efficiency.}
Moreover, we collected proposals on which tasks would be handled using voice assistants. The answers ranged from checking the weather to viewing incoming messages. Generally, users had in mind specific features from their mobile applications that they would like to carry out using voice commands. From the experiment, participants spent a great amount of time reaching the destination screen inside an application to perform the task which underscores the challenges in navigating in the context of voice control. P1 and P6 proposed enhancing the voice assistant’s capability to directly access a feature, as in Google Assistant or Apple Siri, so that they would be able to view specific information or open the desired feature in one command.


\textit{Robustness to the rich linguistic variations in the human command utterances.}
From the experiment, one major issue that caused the inaccuracy of the voice system was the rich linguistic variations in human utterances. Users might describe one action or target using multiple word choices. For example, participants used ``tap'' or ``click'' to perform the action of ``PRESS''. In addition, the application name such as ``Gmail'', might be mentioned as ``Gmail'' or ``Google mail''. The complexity of multiple variations in word choice within a single command caused the existing system to misunderstand the user's intention in their command utterances. As a result, users expressed frustration when undoing the misinterpreted command, which negatively affects the user experience.



\subsection{Design Goals}
Based on the findings in the previous section, we propose the design goals to improve the usability of existing tools: 
\begin{itemize}

  
  \item \textbf{Efficiency:} Provide direct access to in-app features without navigating through multiple screens using voice commands to reduce the time to complete a certain activity.
  \item \textbf{Comprehensibility:} Reduce the learning curve of the system and require minimal cognitive load from users to operate the tool.
  \item \textbf{Robustness:} Understand the user's intention in human speech utterances with rich linguistic variations to avoid misinterpretation of user commands.


\end{itemize}

==> old_content/DesignConcepts.tex <==
\section{Design Concepts}
\label{sec:designConcepts}

Voicify system is built to leverage voice interactions between the user and Android devices. The system extends Google Assistant to open specific features within an application that have not declared the app actions which saves efforts of the app developers. When a user requests to open an unsupported component via Google Assistant, Voicify will capture that request, search for mentioned queries and directly present it. In addition, our system provides a background service, which continuously listens to users’ commands to interact with the on-screen UI elements. The feature includes normal interactions, namely clicking, swiping, entering texts and other navigating actions\han{Can we find a reference say those are the common actions}. Voicify functions completely based on the collected data from the device, hence providing a lightweight, up-to-date personal assistant. The overall system design is demonstrated in Figure~\ref{fig:overview}, we provided an use case of getting  nutritional facts for a healthy burger recipe in World Recipes application.

We identified some important challenges that Voicify will resolve to extend current studies and systems in this field. 

\subsection{Direct Component Invocation}

One of the biggest contributions of Voicify is allowing the cold start of specific components from the outside of certain apps. First, when the user initiates Voicify, a service will fetch all intent patterns and deep links from installed applications, store them in a persistent database. When the user mentions a specific feature along with the application name in Google Assistant, the related intent filters will be retrieved. A priority sorting algorithm will sort these data and invoke the one with the highest priority. Finally, the desired screen will be displayed on the user's device, allowing users to promptly perform their task without navigating through the preceding application's screen. We also allow systematic filtering and validation and manual user modifications to obtain the best match. In Figure  \ref{fig:overview}, Voicify directly provides "My Recipes" screen within World Cuisines application.


\subsection{Virtual Assistant Services}
In addition to the direct invocation of requested features, Voicify also provides state-of-the-art virtual assistant services. On starting Voicify, compact controlling buttons will appear, allowing users to initiate the continuous speech listener to work in the background. On recognizing user commands, the service will promptly extract action-target pairs, performing the action on the specified targeted UI element. Within one utterance, users can specify multiple tasks to be executed respectively. A talk-back system is also integrated, giving feedback to users on task completion.

For virtual assistant services to work, we interpret elements on the active window to extract all interactive elements and find their corresponding texts. This piece of text will be the label for the user to perform interactions on the target. For those interactive elements without any visible text, a tooltip labelling system will assign each of them with a unique number for references. Voicify also implemented a setting page to allow customization on tooltips' characteristics, such as colours, size and opacity.

==> old_content/Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We conducted two experiments to evaluate the effectiveness of our implementation. In the first study, we test the feasibility of the direct component invocation module. We measure this by opening features that has Google Assistant app actions integrated using \tool. In the second study, we requested participants to perform specific tasks using \tool and Voice Access. We released the detailed data and evaluation results in a repository \footnote{\url{https://anonymous.4open.science/r/voicify-evaluation-1B83/}}.
\subsection{Measuring Direct Feature Invocation Precision}

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{assets/testcase.png}
\caption{Example test cases for Message and Twitter application, where direct pages from applications are opened}
\label{fig:testcase}
\end{figure}

\subsubsection{Experiment design}
In this experiment, we validate the ability of \tool to retrieve and directly open a feature from another application. We use Google Assistant as the ground truth of this experiment since it supports direct feature invocation. We come up with a list of features from different applications that can be invoked using Google Assistant~\cite{web:assistantGoogle}. Since developers can declare Google Assistant supported features inside the app action file, we extracted the list of features that each application provides to Google Assistant by analyzing the \emph{actions.xml} file located inside the application package. Out of 6,000 application packages that we collected from Google Play Store, we only found 42 applications that have the \emph{actions.xml} file. We can only gather a small number of applications because applications can also integrate with Google Assistant via the Google Actions Console. However, Google Assistant does not provide a centralized database of supported applications that we can directly extract. Some applications have not correctly declared their \emph{actions.xml} file, therefore causing their integration with Google Assistant to malfunction. In addition, some applications have not updated their Google Assistant declarations according to their feature updates. Due to those reasons, we manually tested each feature that we collected on Google Assistant. As result, we only achieved 32 application features from analysing the \emph{actions.xml} file. We expanded our scope to also achieve Google Supported features from those applications without the \emph{action.xml} declaration. From Play Store, we downloaded some popular applications and manually tested their Google Assistant usage. In the end, we achieved a list of 50 features from 25 applications for our evaluation. We showed an example of 2 test cases in Figure~\ref{fig:testcase}.

After getting the application name and feature name that has Google Assistant supported, we created the user command set. To simulate natural human commands, we used the command patterns that were previously extracted and filtered from Google Assistant. We appended the feature name and application name pairs that were previously extracted into these command patterns to form a complete test case. 
% In addition, we appended our app name so that Google Assistant can trigger our application. 
Finally, the test cases contain 50 commands which have different patterns to open 50 different features. We invoke these commands to validate if the desired feature can be invoked by \tool.



\subsubsection{Metrics}

 As ground truth, we invoked each feature with Google Assistant and recorded the destination screen. In our experiment, we evaluate our approach using the hit rate@k, with k = 1,3. We use k = 1 to imply the feature that will be opened by the direct invocation module. Hit rate at k = 3 represents the top-3 recommended features that can be invoked by \tool. 
 
 In detail, \tool returns a list of related intents that are sorted based on the relevance score and invoke the intent with the highest relevance score. Therefore, we collect the hit rate at k = 1 to record the number of times \tool can invoke the precise intent. Each of the tasks will be marked as successful if our system can provide an identical screen to the ground truth. Using k = 1, we solely evaluate the prioritization system and overall usefulness of the direct invocation module. In addition, we analyse the hit rate at k = 3 to evaluate the ability to retrieve and prioritise features from an application. We marked success for each test case that the ground truth is in included in the top-3 proposed features from \tool.
 
\begin{table}[]
\begin{tabular}{cccc}
\hline
\textbf{Hit rate@k} & \textbf{No of Success} & \textbf{No of Fail} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Percentage\\  of Success\end{tabular}}} \\ \hline
\textit{k = 1} & 38 & 12 & 76\% \\ 
\textit{k = 3} & 41 & 9 & 82\% \\ \hline
\end{tabular}
\caption{The experiment results with k = 1 and k = 3 for 50 test cases.}
\label{table:result}
\end{table}

\subsubsection{Result}

Table~\ref{table:result} demonstrates the result of direct feature invocation evaluation. For k = 3, \tool is able to locate and retrieve 41 corresponding features (82\%). There are 9 features that \tool could not identify (18\%). The failed test cases mostly occur in a small number of applications, which include eBay or Yahoo Finance. The result shows an acceptable performance of the feature retrieval module. For k = 1, we achieved 38 successful test cases out of 50 test cases in total. The average success rate of \tool is 76\%. 
% We achieved high accuracy for the majority of well-known apps, such as Twitter, Yahoo Mail and Aliexpress with 14 out of 16 successful test cases (87.5\%). 
\tool fails to invoke 12 test cases. 

We performed error analysis by investigating each failed test case to understand the causes. First, \tool was unable to map highly abstract commands to application components. For example, ``buy headphones from eBay'' was not executed since \tool cannot interpret the ``buy headphone'' phrase correctly. Second, \tool cannot resolve inconsistencies in the naming convention of Android activity and intent action name within the application, hence causing issues in feature mapping. Third, some activities are not exported by the developer, hence \tool is not able to invoke them outside the app. Forth, the activity that contains the desired feature requires some specified parameters, which we are unable to identify the key and data type required. Fifth, some applications have implemented a centralized activity as the entry point for all external invocations through intent. This implementation limited the list of features that is can be captured by \tool, hence reducing the probability of matching features. In Section~\ref{sec:discussion}, we further discuss how we can improve \tool to address the issues.

Lastly, since \tool aims to address features that are not declared to Google Assistant, our system is capable of opening features that Google Assistant cannot invoke. We found several features that \tool can launch which has not been declared to Google Assistant.


    
    
    
    
  
  
  


==> old_content/Implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\tool system is implemented using Java programming language to work natively in Android OS
~\cite{java_programming_language_2022}. As \tool provides a system-wide voice controlling solution, our app is built on top of many advanced Android developed features, such as voice recognition or accessibility tools. Those features are provided to the developer through application programming interfaces (API) and external packages. In this section, we mentioned four critical concepts within our system and iterated through the implemented technologies.

\subsection{Voice integration \&  command parsing}

\tool is implemented as a voice based application, which allows users to communicate with the device through voice input and audio feedback. We implement two workflows to obtain user voice input and transfer it to text with separated implementations.


  \subsubsection{Invocation through Google Assistant.\\}
  As we aim to leverage the usage of Google Assistant, users can interact with our system via the speech recognition provided by Google. In Android, Google Assistant can only work with apps that have specifically declared its functionalities to the platform. Therefore, the assistant is limited to functionalities that are submitted to them.
  
  In order to declare a feature to Google Assistant, developers create built-in or custom intents. Built-in intent format has been provided by Google Assistant, and developer must adopt the specific format with required parameters. On the other hand, custom intent is recently added, allowing developers to specify their own unique intent with custom command patterns and parameters. Custom intent allows more flexibility and ability to enhance the power of Google Assistant.
  
  Our approach leverages Google Assistant by using the custom intent~\cite{custom_intent_2022} . We created our own intent which requests an app name and a feature name from the user. We extracted the most common commands patterns that are used for opening a specific feature from a large dataset *, and provided them to Google Assistant. When the user's command matches the pattern, Google Assistant will invoke \tool and deliver the parameters to our navigation module, which subsequently open the desired feature on the user's screen. For example in Figure~\ref{fig:overview}, given the command "open Check in page in Service Victoria", Google Assistant will invoke our module, attaching "Check in" as the feature and "Service Victoria" as the app name. A successful invocation will trigger the continuous listener for subsequent on-screen interaction.
  
  \begin{figure}
\centering
\includegraphics[width=\linewidth]{assets/voice.png}
\caption{The Action-Target matching algorithm extracts Action-Target pairs from user commands. It checks for possible synonyms and compares it with the available on-screen target.}
\label{fig:voice}
\end{figure}

  \subsubsection{Interaction with the continuous listener.\\}
 Our main objective is to provide a voice controlling system that can completely replace physical interactions with mobile's screen after taking user to the desired feature within any app. Therefore, in addition to invocation through Google Assistant, we implemented a virtual assistant that continuously listens to users’ commands in the background. This is achieved by integrating Google Speech Recognizer~\cite{speechrecognizer} into a service, which processes the audio input into text format. Given a voice input, \tool system first filters out all unnecessary words in human verbal speech to increase the accuracy of string extraction. After that, we perform character matching to extract all actions presented in the sentence and the succeeding phrase as its target. \tool will create an object that contains this pair of action-target and store it for execution. Additionally, our system also handles common input errors in human verbal communication such as faulty grammar or incorrect usages of articles. We utilize the Synonyms Handler to solve synonym usage in commands. In the system, the Synonyms Handler communicates with a synonyms REST API, retrieves synonymous words for all actions and caches for future usage~\cite{synonyms_api_2022}. For example, an action PRESS can be invoked with its synonyms "click", "tap", "touch", which assists with human natural language. The parsed command’s Action-Target pairs are then delivered to the Action mapping and execution module to be executed. In Figure~\ref{fig:voice}, we demonstrated the overview design of action-target pair extraction module.
 
 Using complex sentence is a natural tendency of human speech, which allows more information to be mentioned within a single sentence. In order to improve the user experience, \tool introduces command chaining, which allowing users to indicate multiple tasks within a single utterance, separated by the "AND" keyword. The system will extract and store all action-target pairs respectively according to the order that user specified. In Figure~\ref{fig:voice}, three action-target pairs has been extracted from user command and stored in the for execution.

\begin{figure*}[!h]
\centering
\includegraphics[width=0.8\textwidth]{assets/extraction.png}
\caption{The extraction algorithm extracts and decodes the retrieved Android-specific binary XML files. It produces a completed list of application's intent filters.}
\label{fig:extraction}
\end{figure*}

\subsection{Intent patterns \& Deep links retrieval}

\tool app utilized on-device data to obtain developed features from installed apps. For direct invocation process, our system requires the deep links or intent patterns to generate an intent messaging object. In addition, we gather the application name and component name for matching with user commands. To retrieve the mentioned piece of information from other applications, we requested the permission GET\_META\_DATA, GET\_SHARED\_LIBRARY\_FILE and QUERY\_ALL\_PACKAGES. In Figure~\ref{fig:extraction}, we have demonstrated the pipeline for extracting all intent filters from retrieved application data. First, we fetch all applications' package names using the Package Manager, which is a system class that provides all information related to packages that are installed on the Android device~\cite{packagemanager}.  This package name is unique to each application and will be used to determine the directory name that stores the application local data. Since app manifest file stores all of the activity names within the app with their corresponding intent filters ,we locate and retrieve the app manifest file from these directories. However, the data is stored as Android-specific binary XML format, allocated into chunks with litter-endian byte order by default and protected by Android system. Therefore, we read the file in stream of bytes and implemented a custom binary decoder to convert the data into UTF-8-character representation. The decoder finally concatenate separated chunks of character and returns the complete application manifest file in a human-readable format (UTF-8) for further data extraction. As deep links and intent patterns are scattered in the extracted Manifest file, we implemented a searching and filtering algorithm to extract all exposed features from apps precisely. As we have mentioned that the intent filter contains required data for constructing intent that can open corresponding feature, the system obtains the data within each \emph{<intent-filter>} tag from the XML file to get all the intent filters. In Figure~\ref{fig:intent}, we have illustrated the representation and retrieval of deep links and intent patterns in the manifest file for YouTube application.

\begin{figure*}[!h]
\centering
\includegraphics[width=0.8\textwidth]{assets/intent.png}
\caption{The hierarchical structure of the manifest file. We extract the required fields by string extraction to form intent object.}
\label{fig:intent}
\end{figure*}

  \subsubsection{Intent patterns}
    Since \tool directly invokes other components via intent-based communication, it is essential to form suitable intents that can trigger the corresponding intent filter. An explicit intent invocation consists of a specific destination that allow the Android system to identify the correct target. The attached destination component includes the package and activity name, which is stated in the manifest. For better granularity of feature exploration, \tool utilizes the declared action name, which is attached to the intent object. A list of common and standard actions is provided by Android and Google for starting specific tasks or features along with developer custom actions~\cite{commonintent}. In the end, the gathered information will be added to the intent and stored for retrieval.

    \subsubsection{Deep links}
    Our aim is to retrieve and form all supported deep links from an application manifest file, hence exploring the set of features created for direct invocation by app developers. Since a deep link can only be invoked from other apps if the holder intent filter's category is set to BROWSABLE and DEFAULT, \tool eliminates those which does not match this requirement. According to Android official documentation \cite{deep_links}, A typical deep link includes a host, scheme and path prefix, which are specified within the \emph{<data>} tag, located in intent filters. The system fetches and concatenates them in sequence to form a complete deep link. We used a validation system that filters out all invalidated and repeated deep links to improve the algorithm's robustness. As a deep link is referred to as a unique resource identifier, an intent that attached a deep link can directly invoke an app component without specifying its activity and package. Lastly, Action VIEW is also attached to populate the UI representation of the desired feature to the user.

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{assets/UI-semantic.png}
\caption{We show an example of a normal UI semantic where interactive elements are extracted. These elements can be invoked using the corresponding texts (elements with visible label) or provided tooltip numbers (element without labels). }
\label{fig:UIsemantic}
\end{figure}
\subsection{UI semantic retrieval}

In \tool, UI semantic retrieval is an essential module that allows the system to identify and locate the UI elements. Similar to Kalysch et al.~\cite{kalysch2018android}, we utilized Android Accessibility Service API to gain a system-level semantic understanding of UI element. According to the Android Accessibility developer guide, the Accessibility API provides information about on-screen elements via Accessibility Node Info objects~\cite{accessibilitynodeinfo} to encapsulate the data of UI components. Since Android’s layout is populated in a hierarchical structure, our system uses the Depth First Search algorithm to explore the element tree. From the collected data, \tool retrieves interactive UI elements, and classifies whether they are clickable, scrollable or editable. Android populates the textual using TextView, in which we use the \emph{getText()} method to extract its content. The extracted label will be appended to the interactive nodes used for matching with the target from users' command. For non-TextView interactive elements, we obtain its label by searching for adjacent TextView element which shares the same parent node, inspired by label searching algorithm by Yang's previous work~\cite{yang2020dothishere}.

In several occasions, an interactive element is not attached with any visible labels on the screen, hence user cannot invoke an UI element by mentioning its label. Following the implementation of Voice Access ~\cite{voice_access}, we provide a tooltip labelling system, where a distinct number is dynamically assigned as a temporary label for unlabeled elements. By using the \emph{Layout Inflater}~\cite{layout_inflater}, we display a number next to the unlabeled UI element by tracking its coordinator on the screen. In this way, users can interact with unlabeled elements on the screen using the given tooltip number. For example in Figure~\ref{fig:UIsemantic}, the "option" button is appended number 1 since it does not have any visible label, in which user can press it by saying "press number 1". \tool also solves the problem of catering wider range of users with visual impairment by allowing runtime customization of tooltips.



\subsection{UI elements matching \& action execution}
   \subsubsection{UI elements matching\\}
     Upon UI semantics retrieval has completed, target mapping takes place whenever receiving the Action-Target pairs from the continuous listener. \tool searches for the mentioned targets in the collected UI labels from on-screen elements. The target matching algorithm splits the target into meaningful words and executes string matching with UI label. We set the target search range from the user command to 50 characters, which is the upper limit that Google allows for app names on the Play Store~\cite{50_chars}. If a target match is not found, alternative synonyms will be used to expand the list of potential matches. After that, we sort them by a given priority score to determine the most related element. This priority score is calculated based on the contextual data, percentage and count of matched keywords. On occasions where \tool could not make the decision between multiple targets, an audio prompt will be delivered to the user to determine the desired UI elements. If the target has been determined, \tool will create a pair of action-target and add it to the waiting queue for execution~\cite{van1976design}.
  
 \subsubsection{Action execution\\}

    The action executor listens to changes in the execution waiting queue. We applied the observer pattern~\cite{gruntz2002java} that allows action executor to get notified when new action-target pair is added. If the queue is not empty, the system pops an action from the queue and performs it on the specific UI element by invoking the \emph{performAction()} method~\cite{accessibilitynodeinfo} on the desired node. Android Accessibility API provides a wide range of system control methods that allows accessibility service developer to have full control over user's device. When an action is completed, it triggers the automated validation which verifies if the action is successfully executed by monitoring the changes in UI semantics. \tool will automatically perform the succeeding action once the preceding action is successfully invoked, which allows command chaining to improve the performance. The app also sends an audio feedback to users as an indication that the system is ready for the next command. Finally, the system can be terminated upon pressing the floating STOP button.

==> old_content/Introduction.tex <==
\section{Introduction}

 
Android smartphones nowadays come with a large touchscreen that allows users to directly interact with on-screen elements. However, physical interactions with the mobile screen are troublesome in many scenarios as researchers have pointed out indisputable problems associated with the touchscreen interactivity. Modern screen sizes are becoming larger~\cite{kim2011effects}, interactions are hindered, requiring users' efforts to reach far-part UI elements. On smaller screen sizes, misclicking is a regular behaviour that happens due to clustered elements and complex usage scenarios~\cite{hu2018user}. Research has also shown that texting via virtual keyboard also negatively affects the corresponding finger muscles and joint angles~\cite{kietrys2015mobile}. In addition, interacting with a touchscreen is a tedious process for users whose hands were occupied (e.g., cooking, holding a baby and training) and those who has temporary or permanent motor impairment ~\cite{zhong_raman_burkhardt_biadsy_bigham_2014}. Under those circumstances, attempting to perform physical interactions on the phone such as tapping or scrolling are extremely inconvenient. Due to the stated issues, users expect a more intuitive method to interact with smart devices.

Nowadays, advanced technologies have fueled the development of virtual assistants, which replace traditional touchscreen interactions with the human voice as input. These systems have a diverse range of functionalities, but in general, they listen to the user commands, map the queries to the set of tasks and execute them. This technology changes how both non-disabled and disabled individuals interact with mobile devices. For non-disabled individuals, voice control offers convenience and efficiency of use, and for disabled users, it offers an accessible option through which to dramatically improve their user experiences. The list of most well-known voice assistants includes Alexa, Siri and Cortana, which are integrated into various smart devices across multiple platforms~\cite{hoy2018alexa}. In Android, Google Assistant~\cite{google_assistant} and Google Voice Access~\cite{voice_access} are the most well-known voice assistants, that provide a predefined set of commands and full device control respectively. 

However, some of the key functionalities are still missing or can be extended further from previous research and products. For example, directly opening a specific page from an app, allows users to launch the app at a specific screen that serves their purposes has not been widely adopted by many other applications. Google Assistant has a fixed list of application features that can be invoked directly (namely App Action), with requirements for extra developers’ efforts. Many apps are missing the required declarations, hence their functionalities cannot be invoked Google Assistant~\cite{arsan2021app}. Secondly, there are currently very few Android voice control applications available to users that offer full control over one’s device. The Voice Access that is introduced by Google, has a very limited number of features and users have reported reliability issues within the system~\cite{voice_access_issue}. Another issue with the aforementioned examples is that they are not open source, which prevents other developers from developing and refining the solutions. Lastly, most listed approaches depend heavily on a massive database of Android applications that require frequent updates. 

This paper introduces \tool, a universal voice control Android application with novel approaches to extend current voice assistant products. The system can be triggered to invoke a specific feature from an installed application directly through Google Assistant, even when the feature is not declared to this platform. We achieved this by fetching available components from the user device's applications. After that, we open these components on user devices. In addition, we integrate a continuous listener in the background that obtains the user's voice commands and executes them. \tool allows users to achieve daily physical interactions with mobile devices completely using voice commands. The set of actions includes opening apps, scrolling, tapping or inputting text. These functionalities work seamlessly and universally as a virtual assistant in the background. Furthermore, users can give several commands within one utterance, the application will execute each command sequentially.

We analysed the ability to open a direct feature from other applications by testing the system on a set of features from different applications. The result shows that \tool is capable of retrieving and opening a wide range of features from many different apps. We also conducted a user experiment to evaluate the system's usability. Overall, users agree that Voicify is consistent and easy to use for real-world scenarios. Lastly, we discuss the potential implication of the system, as well as the future works. To summarize, the contributions of our work include:
\begin{enumerate}
  \item A voice control \& navigation system that replaces physical interaction with mobile devices. This is a universal approach with production-level implementation, utilizing an advanced natural language processing algorithm for resolving synonyms and tolerating human errors.
  \item A lightweight solution that retrieves and decodes runtime installed applications metadata. This data is filtered and extracted to form the database of commands that matches certain pages in on-device applications.
  \item The system enhances Google Assistant by expanding its capability to open a direct feature from an app. Intent-based communication is utilized for direct component invocation.

\end{enumerate}

==> old_content/Voicify.tex <==
\section{The Voicify System}

\tool system is built to leverage voice interactions between the user and Android devices. The system extends Google Assistant to open specific features within an application that have not declared the app actions. Hence, we overcome the limitation in the feature coverage of Google Assistant, minimizing developer efforts to comply their apps to the assistant platform. In addition, our system provides a background service, which continuously listens to users’ commands to interact with the on-screen UI elements. The feature includes normal interactions, namely clicking, swiping, entering texts and other navigating actions. The internal functions are completely based on the collected data from the device, hence providing a lightweight, up-to-date personal assistant. The overall system design is demonstrated in Figure~\ref{fig:overview}, we provided a use case for getting nutritional facts for a healthy burger recipe in the World Cuisines application.

\subsection{Direct Component Invocation}

One of the contributions of \tool is allowing the cold start of specific components from the outside of certain apps. Since we have integrated our app with Google Assistant, users can directly use Voicify to open a feature from any installed applications via voice command through the interface of Google Assistant. As the user mentions a feature within a specific app, \tool opens the most relevant screen from that app. We achieved this by matching the user's commands to the data that we collected from installed applications. To match the most suitable screen, we implemented a priority sorting algorithm that sorts the app data and invokes the one with the highest priority. We also allow systematic filtering and validation and manual user modifications to obtain the best match. In Figure  \ref{fig:overview}, \tool directly invokes the "My Recipes" screen within the World Cuisines application.
\begin{figure*}[!h]
\centering
\includegraphics[width=0.8\textwidth]{assets/extraction.png}
\caption{The extraction algorithm extracts and decodes the retrieved Android-specific binary XML files.}
\label{fig:extraction}
\end{figure*}

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{assets/intent.png}
\caption{The hierarchical structure of the manifest file where we extract the required fields by string extraction to form intent object.}
\label{fig:intent}
\end{figure}
\subsubsection{Integration with Google Assistant}
  As we aim to leverage the usage of Google Assistant, users can interact with our system via the speech recognition provided by Google. In Android, Google Assistant can only work with apps that have specifically declared their functionalities to the platform. Therefore, the assistant is limited to functionalities that are submitted to them.
  
  In order to declare a feature to Google Assistant, developers create built-in or custom intents. Built-in intent formats have been provided by Google Assistant, and the developer must adopt the specified format with the required parameters. On the other hand, custom intent~\cite{custom_intent_2022} is recently added, allowing developers to specify their unique intent with custom command patterns and parameters. Custom intent allows more flexibility and the ability to enhance the power of Google Assistant.
  
  Our approach leverages Google Assistant by using the custom intent. We created our custom intent which requests an app name and a feature name from the user as the parameters. For the command patterns, we run a static analysis on a large command database to extract the most common command patterns that are used for opening a specific feature. We constructed the command database by crawling sample commands from the Google Assistant website~\cite{web:assistantGoogle}, which includes 6,649 unique commands that are commonly used in different apps. We then applied Part of Speech (POS) tagging to the extracted commands which resulted in common command patterns  \footnote{\url{https://anonymous.4open.science/r/voicify-evaluation-1B83/arrays.xml}} when opening certain features inside apps. When the user's command matches the extracted patterns, Google Assistant will invoke \tool and send over the parameters to our navigation module, which subsequently opens the desired feature on the user's screen. For example in Figure~\ref{fig:overview}, given the command "open My Recipes page in World Cuisines on Voicify", Google Assistant will invoke our module, attaching "My Recipes" as the feature and "World Cuisines" as the app name.
  
\subsubsection{Exported components \& Deep links retrieval}
While Google Assistant requires developers to manually declare the app's features, \tool utilized on-device data to obtain developed features from installed apps. Hence, our approach is dynamically compatible with any applications without requiring any further works from application developers. For the direct invocation process, our system requires deep links or exported components to generate an intent messaging object. In addition, we gather the application name and component name for matching with user commands. To retrieve the mentioned piece of information from other applications, system-level permission must be granted, including GET\_META\_DATA, GET\_SHARED\_LIBRARY\_FILE and QUERY\_ALL\_PACKAGES permissions. In Figure~\ref{fig:extraction}, we have demonstrated the pipeline for extracting all intent filters from retrieved application data. First, we fetch all applications' package names using the Package Manager, which is a system class that provides all information related to packages that are installed on the Android device~\cite{packagemanager}. This package name is unique to each application and will be used to determine the directory name that stores the application’s local data. Since the app \emph{Manifest.xml} file stores all of the activity names within the app with their corresponding intent filters, we locate and retrieve the app manifest file from these directories.

In each application directory, the data is encoded in Android-specific binary XML format, allocated into chunks with litter-endian byte order by default and protected by the Android system. Therefore, we read the file in a stream of bytes and implemented a custom binary decoder to convert the data into UTF-8-character representation. The decoder finally concatenates separated chunks of characters and returns the complete application manifest file in a human-readable format (UTF-8) for further data extraction. 

Since deep links and exported activity information are scattered in the extracted Manifest file, we implemented a searching and filtering algorithm to extract all exported features from apps precisely. As we have mentioned that the intent filter contains required data for constructing intent that can open the corresponding feature, the system obtains the data within each \emph{<intent-filter>} tag from the XML file to get all the intent filters. In Figure~\ref{fig:intent}, we have illustrated the representation and retrieval of deep links and exported components in the manifest file for the YouTube application.

If an activity has included a deep link, the system retrieves it by concatenating the host, scheme and path prefix in the \emph{<data>} tag. We used a validation system that filters out all invalidated and repeated deep links to improve the algorithm's robustness. Since a deep link is referred to as a unique resource identifier, an intent that attaches a deep link can directly invoke an app component without specifying its activity and package. In Android, each intent needs to specify the action that it would perform on the destination activity ~\cite{intent}. Since we want to view the screen that contains desired feature, we attached the action VIEW to the intent object.

 For those activities that are not integrated with deep links, we open them by forming an explicit intent, which contains the package name and the activity name. For better granularity of feature exploration, \tool utilizes the declared action name, which is attached to the intent object. A list of common and standard actions is provided by Android and Google for starting specific tasks or features along with developer custom actions~\cite{commonintent}. For example, SEARCH is a standard action that is commonly linked to the search feature within an application.
 
 \subsubsection{Application \& feature matching}
    Upon receiving an intent from Google Assistant for direct invocation, \tool extracts the attached feature and application name. First, the system searches for the application mentioned by the user in the installed application namespace. After identifying the matched application, we search for the feature mentioned in the user's command. 
    
    The system fetches the list of intents that corresponds to the identified application. We identify the feature that is linked to each intent by analyzing the intent's information, including the action name, activity name or deep links. The activity name is declared in the camel case format followed Java naming convention~\cite{java_naming_convention}, hence we split it into separated meaningful words. For deep links, we extract the path prefix since it contains information about the matching feature. For example in Figure~\ref{fig:intent}, the path prefix "browse" identifies the browse screen within YouTube. We append these extracted keywords into a list that will be used for intent searching and prioritizing.
    
    When searching for the relevant features within the app, we utilized the generated keywords for each intent. First, the system created a list of intents in which the desired feature appeared in the keywords. After that, we used the number and percentage of matched keywords to give each intent a relevance score. From experiments, we observe that the deep link approach has higher accuracy while exported component invocation has higher coverage. Hence, we give any intent that contains a deep link bonus relevant score. Finally, we achieved the sorted list of intents based on their relevance to the requested feature and invoke the most relevant intent. On occasion when none of the intents that we generated match the specified feature, we open the application entry screen as a baseline. 






 \begin{figure}
\centering
\includegraphics[width=\linewidth]{assets/voice.png}
\caption{The Action-Target matching algorithm extracts Action-Target pairs from user commands. It checks for possible synonyms and compares it with the available on-screen target.}
\label{fig:voice}
\end{figure}


\subsection{Virtual Assistant Services}
Our main objective is to provide a voice controlling system that can completely replace physical interactions with the mobile's screen after taking users to the desired feature within any app. Therefore, in addition to direct component invocation, we implemented a virtual assistant that allows users to finish the rest of their tasks using voice commands. We retrieve UI elements for interaction using Accessibility Service API. On recognizing user commands, the service will promptly extract action-target pairs, performing the action on the specified targeted UI element. Within one utterance, users can specify multiple tasks to be executed respectively. A talk-back system is also integrated, giving feedback to users on task completion.

  \subsubsection{Interaction with the continuous listener}
  To obtain user voice command, we integrated Google Speech Recognizer~\cite{speechrecognizer} into a service, which processes the audio input into text format. Given a voice input, \tool first filters out all unnecessary words in human verbal speeches to increase the accuracy of string extraction. Additionally, our system also handles common input errors in human verbal communication such as faulty grammar or incorrect usage of articles. After that, we perform character matching to extract all actions presented in the sentence and the succeeding phrase as its target. \tool creates an object that contains this pair of action-target and store it for execution. We utilize the Synonyms Handler to solve synonym usage in commands. In the system, the Synonyms Handler communicates with a synonyms REST API, retrieves synonymous words for all actions and caches for future usage~\cite{synonyms_api_2022}. For example, an action PRESS can be invoked with its synonyms "click", "tap", "touch", which assists with human natural language. The parsed command’s Action-Target pairs are then delivered to the Action mapping and execution module to be executed. In Figure~\ref{fig:voice}, we demonstrated the overview design of the action-target pair extraction module.
 
 Using complex sentences is a natural tendency of human speech, which allows more information to be mentioned within a single sentence. In order to improve the user experience, \tool introduces command chaining, which allows users to indicate multiple tasks within a single utterance, separated by the "AND" or "THEN" keyword. The system will extract and store all action-target pairs respectively according to the order that the user specifies. In Figure~\ref{fig:voice}, three action-target pairs have been extracted from the user command and stored for execution.



\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{assets/UI-semantic.png}
\caption{We show an example of a normal UI semantic where interactive elements are extracted. These elements can be invoked using the corresponding texts (elements with visible label) or provided tooltip numbers (element without labels). }
\label{fig:UIsemantic}
\end{figure}

\subsubsection{UI semantic retrieval}
In \tool, UI semantic retrieval is an essential module that allows the system to identify and locate the UI elements for interactions. Similar to Kalysch et al.~\cite{kalysch2018android}, we utilized Android Accessibility Service API to gain a system-level semantic understanding of UI elements. According to the Android Accessibility developer guide, the Accessibility API provides information about on-screen elements via Accessibility Node Info objects~\cite{accessibilitynodeinfo} to encapsulate the data of UI components. Since Android’s layout is populated in a hierarchical structure, our system uses the Depth First Search algorithm to explore the element tree. From the collected data, \tool retrieves interactive UI elements and classifies whether they are clickable, scrollable or editable. Android populates the textual using TextView, in which we use the \emph{getText()} method to extract its content. The extracted label will be appended to the interactive nodes used for matching with the target from the users' command. For non-TextView interactive elements, we obtain its label by searching for adjacent TextView element which shares the same parent node, inspired by the label searching algorithm in Yang's previous work~\cite{yang2020dothishere}.

On several occasions, an interactive element is not attached with any visible labels on the screen, hence the user cannot invoke a UI element by mentioning its label. Following the implementation of Voice Access ~\cite{voice_access}, we provide a tooltip labelling system, where a distinct number is dynamically assigned as a temporary label for unlabeled elements. By using the \emph{Layout Inflater}~\cite{layout_inflater}, we display a number next to the unlabeled UI element by tracking its coordinator on the screen. In this way, users can interact with unlabeled elements on the screen using the given tooltip number. For example in Figure~\ref{fig:UIsemantic}, the "option" button is appended number 1 since it does not have any visible label, in which user can press it by saying "press number 1". \tool also solves the problem of catering wider range of users with visual impairment by allowing runtime customization of tooltips. Users can change all the aspects of tooltips' appearance, including the size, colour and opacity.

\subsubsection{UI elements matching \& action execution}
     Target mapping takes place upon receiving the Action-Target pairs from the continuous listener. \tool searches for the mentioned targets in the collected UI labels from on-screen elements. The target matching algorithm splits the target into meaningful words and executes string matching with the UI label. We set the target search range from the user command to 50 characters, which is the upper limit that Google allows for app names on the Play Store~\cite{50_chars}. If a target match is not found, alternative synonyms will be used to expand the list of potential matches. After that, we sort them by a given priority score to determine the most related element. This priority score is calculated based on the contextual data, percentage and count of matched keywords. On occasions where \tool cannot decide between multiple targets, an audio prompt will be delivered to the user to determine the desired UI elements. If the target has been determined, \tool will create a pair of action-target and add it to the waiting queue for execution~\cite{van1976design}.

    The action executor listens to changes in the execution queue. We applied the observer pattern~\cite{gruntz2002java} that allows the action executor to get notified when new action-target pair is added. If the queue is not empty, the system pops an action from the queue and performs it on the specific UI element by invoking the \emph{performAction()} method~\cite{accessibilitynodeinfo} on the desired node. Android Accessibility API provides a wide range of system control methods that allows accessibility service developer to have full control over users’ device. When an action is completed, it triggers the automated validation system which verifies if the action is executed by monitoring the changes in UI semantics.  \tool will automatically perform the succeeding action once the preceding action is successfully invoked, which allows command chaining to improve the performance. The app also sends audio feedback to users as an indication that the system is ready for the next command.

\subsection{Implementation}

We used Python scripts to extract common patterns in human commands. We passed this data along with our custom intent by declaring the required XML code. We implemented the application and accessibility background service in Android using Java. Since our filtering and command matching algorithm is executed in runtime, we implemented it using Java.


==> old_content/draft.tex <==
    Exact string matching technique is not adequate for identifying app name since pronouncing an application name is troublesome in some scenarios. The problem arises when applications are known for multiple names (e.g. Google Play Store is also called Google Play or Play Store, Facebook Messenger's official Android app name is Messenger). In addition, some applications are not named using lexical English words, which caused difficulties for the speech recognizer to produce the corresponding written form. This is a well-known issue that has been reported for Google Assistant, which blocked many applications from voice interaction on the platform. We attached a set of heuristics to mitigate the penalties for common issues, including plural usages, missing common words or speech recognizer issues.
    
    
    Identifying the most suitable feature is a challenging task since the information about features are totally dependent on the naming convention used by the developer.  . Therefore, we create a Word2Vec model that can understand high-level natural language to perform similarity comparison between spoken feature name and the generated set of keywords for the recognized features. We trained the model using multiple dataset that specialized in natural language commands to interact with Android devices and applications. The first dataset is the written instructions collected from the AndroidHowTo dataset, including short-form human commands to perform specific tasks on Android devices. In addition, we trained the model using the free-form natural language tasks from MoTIF dataset to improve the ability to recognize application features from human commands. Some feature names may contains multiple words, such as "Log in" or "Privacy Settings". Therefore, we extend the Word2Vec model with n-gram word embedding for frequent phrases that are extracted from the training dataset. When these phrases are identified inside the human commands or the list of features, the included words will be concatenated using a special character to be treated as a single word by the model.
    
    After that, \tool fetches the list of intents that corresponds to the identified application. We identify the feature that is linked to each intent by analyzing intent’s information, including the action name, activity name or deep links. The activity name is declared in the camel case format followed Java naming convention [13], thus, we split it into separated meaningful words. For deep links, we extract the path prefix since it contains information about the matching feature. For example in Figure ??, the path prefix "browse" identifies the browse screen within YouTube. We append these extracted keywords into a list that will be used for intent searching and prioritizing. 
     
    
    When searching for the relevant features within the app, we utilized the generated keywords for each intent. The model gives each intent a similarity score based on the attached set of keywords. From experiments, we observe that the deep link approach has higher accuracy while exported component invocation has higher coverage. Hence, we give any intent that contains a deep link bonus score. Finally, we invoke the feature with highest similarity score by sending the formed intent messaging object.
